Pan-STARRS and PESSTO search for an optical counterpart to the LIGO gravitational wave source GW150914

We searched for an optical counterpart to the first gravitational wave source discovered by LIGO (GW150914), using a combination of the Pan-STARRS1 wide-field telescope and the PESSTO spectroscopic follow-up programme. As the final LIGO sky maps changed during analysis, the total probability of the source being spatially coincident with our fields was finally only 4.2 per cent. Therefore we discuss our results primarily as a demonstration of the survey capability of Pan-STARRS and spectroscopic capability of PESSTO. We mapped out 442 square degrees of the northern sky region of the initial map. We discovered 56 astrophysical transients over a period of 41 days from the discovery of the source. Of these, 19 were spectroscopically classified and a further 13 have host galaxy redshifts. All transients appear to be fairly normal supernovae and AGN variability and none is obviously linked with GW150914. We illustrate the sensitivity of our survey by defining parameterised lightcurves with timescales of 4, 20 and 40 days and use the sensitivity of the Pan-STARRS1 images to set limits on the luminosities of possible sources. The Pan-STARRS1 images reach limiting magnitudes of i = 19.2, 20.0 and 20.8 respectively for the three timescales. For long timescale parameterised lightcurves (with FWHM=~40d) we set upper limits of M_i <= -17.2 -0.9/+1.4 if the distance to GW150914 is D = 400 +/- 200Mpc. The number of type Ia SN we find in the survey is similar to that expected from the cosmic SN rate, indicating a reasonably complete efficiency in recovering supernova like transients out to D = 400 +/- 200 Mpc.

==> table_alltransients.tex <==
\begin{center}
\begin{tabular}{ l l l l l l l p{1cm} }
\hline \hline
Name & RA (J2000) & Dec (J2000) & Disc. Date & Disc. MJD & Disc Mag & filter & Notes \\ \hline
PS15cbm & 08 49 19.85 & +03 48 17.8 & 20150917.62 & 57282.62 & 18.55 & i & \\
PS15ccw & 08 57 30.60 & +04 31 56.1 & 20150917.63 & 57282.63 & 19.31 & i & \\
PS15cci & 09 13 22.76 & +06 10 47.3 & 20150919.63 & 57284.63 & 18.32 & i & \\
PS15ccx & 08 18 03.91 & +04 18 04.2 & 20150919.63 & 57284.63 & 19.42 & z & \\
PS15ccv & 08 55 23.05 & +04 41 19.0 & 20150922.62 & 57287.62 & 20.03 & i & \\
PS15cel & 09 34 11.58 & +05 46 45.2 & 20150923.63 & 57288.63 & 19.53 & i & \\
PS15cki & 09 28 27.24 & +08 00 51.5 & 20150923.64 & 57288.64 & 19.17 & z & \\
PS15cej & 09 35 19.41 & +10 11 50.7 & 20151002.62 & 57297.62 & 18.13 & i & \\
PS15cek & 09 36 41.04 & +10 14 16.2 & 20151002.63 & 57297.63 & 17.24 & z & \\
PS15cke & 09 52 35.14 & -07 36 32.0 & 20151002.64 & 57297.64 & 16.72 & z & \\
PS15ckf & 09 45 57.71 & +09 58 31.4 & 20151003.65 & 57298.65 & 17.57 & y & \\
PS15cwj & 09 27 44.89 & +08 31 32.1 & 20151013.60 & 57308.60 & 20.02 & i & \\
PS15cwi & 09 21 31.27 & +05 10 26.8 & 20151013.61 & 57308.61 & 20.43 & i & \\
PS15ckm & 09 43 47.15 & -02 10 13.3 & 20151013.61 & 57308.61 & 19.57 & i & \\
PS15ckj & 10 07 58.59 & -02 29 47.9 & 20151013.61 & 57308.61 & 18.31 & i & \\
PS15cko & 10 14 01.69 & -06 30 46.9 & 20151013.62 & 57308.62 & 19.51 & i & \\
PS15ckh & 09 24 55.83 & +02 19 25.1 & 20151013.62 & 57308.62 & 19.40 & i & \\
PS15cvz & 10 05 41.49 & +01 05 33.2 & 20151013.62 & 57308.62 & 19.55 & i & \\
PS15cvy & 10 01 45.13 & -00 36 06.8 & 20151013.63 & 57308.63 & 19.76 & i & \\
PS15ckn & 10 13 29.31 & -10 00 06.1 & 20151014.62 & 57309.62 & 19.44 & i & \\
PS15ckk & 10 08 48.60 & -09 54 50.7 & 20151014.62 & 57309.62 & 16.43 & i & \\
PS15dfs & 09 21 37.60 & +12 01 38.0 & 20151015.60 & 57310.60 & 20.94 & i & \\
PS15dfr & 09 18 29.04 & +11 40 10.4 & 20151015.60 & 57310.60 & 21.31 & i & \\
PS15cwm & 09 30 01.03 & +06 58 12.6 & 20151015.61 & 57310.61 & 20.90 & i & \\
PS15dfy & 09 52 48.76 & +06 38 04.5 & 20151015.61 & 57310.61 & 19.82 & i & \\
PS15cvv & 09 49 30.25 & -01 36 37.5 & 20151015.62 & 57310.62 & 20.14 & i & \\
PS15cmr & 09 57 03.59 & -03 53 24.3 & 20151015.62 & 57310.62 & 19.35 & i & \\
PS15cmq & 09 48 22.97 & -03 27 41.4 & 20151015.62 & 57310.62 & 20.19 & i & \\
PS15cvx & 09 54 35.48 & -04 07 22.3 & 20151015.62 & 57310.62 & 20.32 & i & \\
PS15dfv & 09 41 38.31 & -02 10 21.8 & 20151015.62 & 57310.62 & 20.83 & i & \\
PS15cwa & 10 13 18.75 & -10 54 43.9 & 20151015.63 & 57310.63 & 20.27 & i & \\
PS15cwk & 10 13 55.42 & -12 52 49.2 & 20151015.63 & 57310.63 & 20.11 & i & \\
PS15cms & 09 58 35.10 & +00 44 34.7 & 20151017.62 & 57312.62 & 19.93 & i & \\
PS15cvw & 09 52 09.25 & +07 26 48.3 & 20151018.61 & 57313.61 & 19.86 & i & \\
PS15cmp & 08 54 24.40 & +03 54 00.5 & 20151019.58 & 57314.58 & 21.82 & r & \\
PS15crh & 08 51 16.19 & +04 03 57.9 & 20151019.58 & 57314.58 & 21.39 & r & \\
PS15cwh & 08 54 15.18 & +03 04 59.0 & 20151019.58 & 57314.58 & 22.09 & r & \\
PS15cri & 09 36 50.66 & +02 31 20.0 & 20151021.60 & 57316.60 & 20.67 & i & \\
PS15cwb & 10 16 21.58 & -11 00 10.5 & 20151021.61 & 57316.61 & 20.25 & i & \\
PS15dgc & 10 18 20.86 & -10 31 28.3 & 20151021.61 & 57316.61 & 20.42 & i & \\
PS15cwe & 10 10 24.74 & -09 33 10.0 & 20151021.63 & 57316.63 & 20.47 & i & \\
PS15crk & 10 30 03.48 & -17 31 38.7 & 20151021.63 & 57316.63 & 19.97 & i & \\
PS15dgb & 10 04 43.54 & -15 00 03.8 & 20151021.63 & 57316.63 & 20.71 & i & \\
PS15dga & 10 04 42.37 & -09 31 14.8 & 20151021.63 & 57316.63 & 20.34 & i & \\
PS15dfx & 09 50 52.07 & -04 09 46.3 & 20151023.60 & 57318.60 & 20.80 & i & \\
PS15cwg & 10 19 19.55 & -09 16 01.2 & 20151023.61 & 57318.61 & 20.39 & i & \\
PS15crj & 09 42 42.16 & +02 18 09.8 & 20151023.62 & 57318.62 & 20.88 & i & \\
PS15dfz & 09 54 59.64 & +04 14 08.1 & 20151023.62 & 57318.62 & 20.68 & i & \\
PS15dfu & 09 34 24.28 & +06 48 01.0 & 20151023.62 & 57318.62 & 21.19 & i & \\
PS15dft & 09 33 09.38 & +10 28 02.2 & 20151023.62 & 57318.62 & 19.41 & i & \\
PS15dfw & 09 44 11.65 & +04 54 52.1 & 20151024.60 & 57319.60 & 21.00 & i & \\
PS15cwc & 09 59 01.22 & -03 48 04.3 & 20151024.61 & 57319.61 & 21.11 & i & \\
PS15cqx & 10 05 03.70 & -06 29 44.7 & 20151024.61 & 57319.61 & 20.32 & i & \\
PS15dgd & 10 27 26.07 & -14 58 20.1 & 20151024.61 & 57319.61 & 20.55 & i & \\
PS15cqw & 09 45 06.43 & +01 17 02.0 & 20151025.60 & 57320.60 & 20.99 & i & \\
PS15cwd & 10 08 06.70 & -14 25 08.5 & 20151025.62 & 57320.62 & 20.93 & i & \\
\hline
\end{tabular}
\end{center}
